An Empirical Exploration of Curriculum Learning for Neural Machine Translation

Machine translation systems based on deep neural networks are expensive to train. Curriculum learning aims to address this issue by choosing the order in which samples are presented during training to help train better models faster. We adopt a probabilistic view of curriculum learning, which lets us flexibly evaluate the impact of curricula design, and perform an extensive exploration on a German-English translation task. Results show that it is possible to improve convergence time at no loss in translation quality. However, results are highly sensitive to the choice of sample difficulty criteria, curriculum schedule and other hyperparameters.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We introduced a probabilistic view of curriculum learning to evaluate the impact of ordering training samples for neural machine translation within the constraints of existing data organization techniques (such as bucketing and mini-batching).  Our implementation lets us flexibly compare the impact of different sample difficulty criteria and curriculum schedules.

We find that curriculum learning can improve convergence speed without loss in translation quality, as hypothesized in the original curriculum learning approach by \citet{BengioLouradourCollobertWeston2009}. However, our results suggest that curriculum learning should not be limited to the idea of training on easy samples first: curriculum schedules that emphasize difficult samples can also yield convergence speedups. Unfortunately, curriculum learning is highly sensitive to hyperparameter settings, which makes it hard to define best practices to adopt for NMT. 

Our open-source implementation will enable further exploration in a wider range of settings in the future. In particular, it remains to be seen whether curriculum learning behavior is more consistent in tasks where there is a more natural definition of sample difficulty, such as domain adaptation.\marine{not sure whether or not to mention adaptation.}


